All in One: Exploring Unified Video-Language Pre-training

Mainstream Video-Language Pre-training models \cite{actbert,clipbert,violet} consist of three parts, a video encoder, a text encoder, and a video-text fusion Transformer. They pursue better performance via utilizing heavier unimodal encoders or multimodal fusion Transformers, resulting in increased parameters with lower efficiency in downstream tasks. In this work, we for the first time introduce an end-to-end video-language model, namely \textit{all-in-one Transformer}, that embeds raw video and textual signals into joint representations using a unified backbone architecture. We argue that the unique temporal information of video data turns out to be a key barrier hindering the design of a modality-agnostic Transformer. To overcome the challenge, we introduce a novel and effective token rolling operation to encode temporal representations from video clips in a non-parametric manner. The careful design enables the representation learning of both video-text multimodal inputs and unimodal inputs using a unified backbone model. Our pre-trained all-in-one Transformer is transferred to various downstream video-text tasks after fine-tuning, including text-video retrieval, video-question answering, multiple choice and visual commonsense reasoning. State-of-the-art performances with the minimal model FLOPs on nine datasets demonstrate the superiority of our method compared to the competitive counterparts. The code and pretrained model have been released in https://github.com/showlab/all-in-one.

==> figures/4-Patch_Visualization.tex <==
\begin{figure}[t]
  \centering
    \includegraphics[width=.85\linewidth]{figures/src/patch_distribution.pdf}
   \caption{
   The patch distribution over.
   }
   \label{fig:4_patch_distribution}
\end{figure}



==> figures/img_parallel_example.tex <==
\begin{figure}[t]
    \centering\small
    \begin{minipage}[t!]{0.57\textwidth}
        \centering\small
        \includegraphics[width=0.85\columnwidth]{figures/nms_fig4.pdf}
        \caption{%
        }
        \label{fig:main_ppl}
    \end{minipage}
    \hskip1em
    \begin{minipage}[t!]{0.35\textwidth}
        \centering\small
        \vskip0.8em
        \includegraphics[width=\columnwidth]{figures/giraffe_collage2.jpg}
        \vskip0.8em
        \caption{%
        }
        \label{fig:token_roll_layer}
    \end{minipage}
\end{figure}

==> tables/abl_initalize.tex <==
\begin{table}\centering
{
\scalebox{\GlobalTableRescale}
{
\begin{tabular}{l|c|r}
Initialize&Steps & Accuracy\\
\shline
 &8& 81.7	\\
 &16& 82.9 \\
\hline
- &200K & \bf  \\
- &800K & \bf  \\
ImageNet&200K& \bf 56.3  \\
ImageNet-21K&200K& \bf 56.3  \\
\end{tabular}
}
}
\caption{Comparison with different initialization for \ModelNameBase.}
\label{tab:abl_initalie}
\end{table}

==> tables/table_test.tex <==
\begin{table}[!tb]
\centering
\scriptsize
\caption{\small Per-facet comparisons between MUFI and training/fine-tuning the network by considering one facet after another.}
%\begin{tabularx}{0.48\textwidth}
\begin{tabularx}{0.88\textwidth}{X|c@{~~~~}c@{~~~~}c@{~~~~}c@{~~~~}c@{~~~~}c|c}
\toprule
\textbf{Method} & \textbf{act.} & \textbf{eve.} & \textbf{int.} & \textbf{spo.} & \textbf{obj.} & \textbf{sce.} & \textbf{avg} \\
\midrule
K700 & 57.6 & 17.9 & 17.8 & 53.1 & 74.2 & 93.1 & 52.2 \\
K700+MIT & 45.0 & \textbf{27.3} & 16.6 & 47.6 & 70.0 & 94.8 & 50.2 \\
K700+MIT+SSV2 & 21.7 & 9.1 & 39.7 & 28.0 & 43.7 & 64.2 & 34.4 \\
K700+MIT+SSV2+S1M & 35.7 & 18.2 & 12.3 & \textbf{68.8} & 69.2 & 88.2 & 48.7 \\ \midrule
\textbf{MUFI} & \textbf{57.8} & 27.0 & \textbf{47.8} & 67.7 & \textbf{77.8} & \textbf{97.5} & \textbf{62.6} \\
\bottomrule
\end{tabularx}
\label{tab:iterative}
\vspace{-0.2in}
\end{table}
